Discovery of X-ray polarization angle rotation in active galaxy Mrk 421

The magnetic field conditions in astrophysical relativistic jets can be probed by multiwavelength polarimetry, which has been recently extended to X-rays. For example, one can track how the magnetic field changes in the flow of the radiating particles by observing rotations of the electric vector position angle $\Psi$. Here we report the discovery of a $\Psi_{\mathrm x}$ rotation in the X-ray band in the blazar Mrk 421 at an average flux state. Across the 5 days of Imaging X-ray Polarimetry Explorer (IXPE) observations of 4-6 and 7-9 June 2022, $\Psi_{\mathrm x}$ rotated in total by $\geq360^\circ$. Over the two respective date ranges, we find constant, within uncertainties, rotation rates ($80 \pm 9$ and $91 \pm 8 ^\circ/\rm day$) and polarization degrees ($\Pi_{\mathrm x}=10\%\pm1\%$). Simulations of a random walk of the polarization vector indicate that it is unlikely that such rotation(s) are produced by a stochastic process. The X-ray emitting site does not completely overlap the radio/infrared/optical emission sites, as no similar rotation of $\Psi$ was observed in quasi-simultaneous data at longer wavelengths. We propose that the observed rotation was caused by a helical magnetic structure in the jet, illuminated in the X-rays by a localized shock propagating along this helix. The optically emitting region likely lies in a sheath surrounding an inner spine where the X-ray radiation is released.

==> norev_author_list.tex <==
\author[1]{Laura Di Gesu}
\author[2]{Herman L. Marshall}
\author[3]{Steven R. Ehlert}
\author[4,5,6]{Dawoon E. Kim}
\author[1]{Immacolata Donnarumma}
\author[7]{Fabrizio Tavecchio}
\author[8]{Ioannis Liodakis}
\author[9,10]{Sebastian Kiehlmann}
\author[11]{Iv\'{a}n Agudo}
\author[12,13]{Svetlana G. Jorstad}
\author[4]{Fabio Muleri}
\author[12]{Alan P. Marscher}
\author[14]{Simonetta Puccetti}
\author[14,15]{Riccardo Middei}
\author[14,15]{Matteo Perri}
\author[4]{Luigi Pacciani}
\author[16,17,18]{Michela Negro}
\author[19]{Roger W. Romani}
\author[4]{Alessandro Di Marco}
\author[9,10]{Dmitry Blinov}
\author[10]{Ioakeim G. Bourbah}
\author[10]{Evangelos Kontopodis}
\author[9,10]{Nikos Mandarakas}
\author[9,10]{Stylianos Romanopoulos}
\author[20,9,10]{Raphael Skalidis}
\author[10]{Anna Vervelaki}
\author[9,10]{Carolina Casadio}
\author[11]{Juan Escudero}
\author[21]{Ioannis Myserlis}
\author[22]{Ramprasad Rao}
\author[22]{Mark Gurwell}
\author[22]{Garrett K.~Keating}
\author[8]{Pouya M. Kouch}
\author[8]{Elina Lindfors}
\author[11]{Francisco Jos\'{e} Aceituno}
\author[11]{Maria I. Bernardos}
\author[7,11]{Giacomo Bonnoli}
\author[11]{V\'{i}ctor Casanova}
\author[11]{Maya Garc\'{i}a-Comas}
\author[11]{Beatriz Ag\'{i}s-Gonz\'{a}lez}
\author[11]{C\'{e}sar Husillos}
\author[23]{Alessandro Marchini}
\author[11]{Alfredo Sota}
\author[24]{Ryo Imazawa}
\author[25]{Mahito Sasada}
\author[24,26,27]{Yasushi Fukazawa}
\author[24,26,27]{Koji S Kawabata}
\author[24,26,27]{Makoto Uemura}
\author[26]{Tsunefumi Mizuno}
\author[26]{Tatsuya Nakaoka}
\author[28]{Hiroshi Akitaya}
\author[29]{George A. Borman}
\author[29]{Alexey V. Zhovtan}
\author[11]{Jos\'{e} L. G\'{o}mez}
\author[15,14]{Lucio A. Antonelli}
\author[30]{Thibault Barnounin}
\author[31,32]{Raffaella Bonino}
\author[1]{Elisabetta Cavazzuti}
\author[1]{Luigi Costamante}
\author[33]{Chien-Ting Chen}
\author[32,31]{Nicol\`{o} Cibrario}
\author[4]{Alessandra De Rosa}
\author[31]{Federico Di Pierro}
\author[21]{Manel Errando}
\author[3]{Philip Kaaret}
\author[34]{Vladimir Karas}
\author[35]{Henric Krawczynski}
\author[35]{Lindsey Lisalda}
\author[19]{Grzegorz Madejski}
\author[36]{Christian Malacaria}
\author[30]{Fr\'ed\'eric Marin}
\author[1]{Andrea Marinucci}
\author[31,32]{Francesco Massaro}
\author[37]{Giorgio Matt}
\author[38]{Ikuyuki Mitsuishi}
\author[3]{Stephen L. O'Dell}
\author[32]{Alessandro Paggi}
\author[19]{Abel L. Peirson}
\author[39]{Pierre-Olivier Petrucci}
\author[3]{Brian D. Ramsey}
\author[3]{Allyn F. Tennant}
\author[40]{Kinwah Wu}
\author[41]{Matteo Bachetti}
\author[42,43]{Luca Baldini}
\author[3]{Wayne H. Baumgartner}
\author[42]{Ronaldo Bellazzini}
\author[37]{Stefano Bianchi}
\author[3]{Stephen D. Bongiorno}
\author[42]{Alessandro Brez}
\author[44,45,46]{Niccol\`{o} Bucciantini}
\author[4]{Fiamma Capitanio}
\author[42]{Simone Castellano}
\author[47,14]{Stefano Ciprini}
\author[4]{Enrico Costa}
\author[4]{Ettore Del Monte}
\author[19]{Niccol\`{o} Di Lalla}
\author[48]{Victor Doroshenko}
\author[34]{Michal Dov\v{c}iak}
\author[49]{Teruaki Enoto}
\author[4]{Yuri Evangelista}
\author[4]{Sergio Fabiani}
\author[4]{Riccardo Ferrazzoli}
\author[50]{Javier A. Garcia}
\author[51]{Shuichi Gunji}
\author[52]{Kiyoshi Hayashida}
\author[53]{Jeremy Heyl}
\author[54]{Wataru Iwakiri}
\author[49]{Takao Kitaguchi}
\author[3]{Jeffery J. Kolodziejczak}
\author[4]{Fabio La Monaca}
\author[31]{Luca Latronico}
\author[31]{Simone Maldera}
\author[42]{Alberto Manfreda}
\author[55]{C.-Y. Ng}
\author[19]{Nicola Omodei}
\author[31]{Chiara Oppedisano}
\author[15]{Alessandro Papitto}
\author[56]{George G. Pavlov}
\author[42]{Melissa Pesce-Rollins}
\author[41]{Maura Pilia}
\author[41]{Andrea Possenti}
\author[57]{Juri Poutanen}
\author[4]{John Rankin}
\author[4]{Ajay Ratheesh}
\author[33]{Oliver Roberts}
\author[42]{Carmelo Sgr\`{o}}
\author[22]{Patrick Slane}
\author[4]{Paolo Soffitta}
\author[42]{Gloria Spandre}
\author[33]{Doug Swartz}
\author[49]{Toru Tamagawa}
\author[58]{Roberto Taverna}
\author[38]{Yuzuru Tawara}
\author[3]{Nicholas E. Thomas}
\author[6,47,59]{Francesco Tombesi}
\author[41]{Alessio Trois}
\author[57]{Sergey S. Tsygankov}
\author[58,40]{Roberto Turolla}
\author[60]{Jacco Vink}
\author[3]{Martin C. Weisskopf}
\author[61,4]{Fei Xie}
\author[40]{Silvia Zane}
%\cortext[corr]{Corresponding author}
\affil[1]{ASI \-Agenzia Spaziale Italiana, Via del Politecnico snc, 00133 Roma, Italy}
\affil[2]{MIT Kavli Institute for Astrophysics and Space Research, Massachusetts Institute of Technology, 77 Massachusetts Avenue, Cambridge, MA 02139, USA}
\affil[3]{NASA Marshall Space Flight Center, Huntsville, AL 35812, USA}
\affil[4]{INAF Istituto di Astrofisica e Planetologia Spaziali, Via del Fosso del Cavaliere 100, 00133 Roma, Italy}
\affil[5]{Dipartimento di Fisica, Universit\`{a} degli Studi di Roma \virg{La Sapienza}, Piazzale Aldo Moro 5, I\-00185 Roma, Italy}
\affil[6]{Dipartimento di Fisica, Universit\`a degli Studi di Roma \virg{Tor Vergata}, Via della Ricerca Scientifica 1, 00133 Roma, Italy}
\affil[7]{INAF Osservatorio Astronomico di Brera, Via E. Bianchi 46, 23807 Merate (LC), Italy}
\affil[8]{Finnish Centre for Astronomy with ESO,Â  20014 University of Turku, Finland}
\affil[9]{Institute of Astrophysics, Foundation for Research and Technology-Hellas, GR-71110 Heraklion, Greece}
\affil[10]{Department of Physics, University of Crete, 70013, Heraklion, Greece}
\affil[11]{Instituto de Astrof\'{i}sica de Andaluc\'{i}a-CSIC, Glorieta de la Astronom\'{i}a s/n, 18008, Granada, Spain}
\affil[12]{Institute for Astrophysical Research, Boston University, 725 Commonwealth Avenue, Boston, MA 02215, USA}
\affil[13]{Department of Astrophysics, St. Petersburg State University, Universitetsky pr. 28, Petrodvoretz, 198504 St. Petersburg, Russia}
\affil[14]{Space Science Data Center, Agenzia Spaziale Italiana, Via del Politecnico snc, 00133 Roma, Italy}
\affil[15]{INAF Osservatorio Astronomico di Roma, Via Frascati 33, 00078 Monte Porzio Catone (RM), Italy}
\affil[16]{University of Maryland, Baltimore County, Baltimore, MD 21250, USA}
\affil[17]{NASA Goddard Space Flight Center, Greenbelt, MD 20771, USA}
\affil[18]{Center for Research and Exploration in Space Science and Technology, NASA/GSFC, Greenbelt, MD 20771, USA}
\affil[19]{Department of Physics and Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, Stanford, California 94305, USA}
\affil[20]{Owens Valley Radio Observatory, California Institute of Technology, MC 249-17, Pasadena, CA 91125, USA}
\affil[21]{Institut de Radioastronomie Millim\'{e}trique, Avenida Divina Pastora, 7, Local 20, E\-18012 Granada, Spain}
\affil[22]{Center for Astrophysics $\vert$ Harvard \& Smithsonian, 60 Garden St, Cambridge, MA 02138, USA}
\affil[23]{University of Siena, Astronomical Observatory, Via Roma 56, 53100 Siena, Italy}
\affil[24]{Department of Physics, Graduate School of Advanced Science and Engineering, Hiroshima University Kagamiyama, 1-3-1 Higashi-Hiroshima, Hiroshima 739-8526, Japan}
\affil[25]{Department of Physics, Tokyo Institute of Technology, 2-12-1 Ookayama, Meguro-ku, Tokyo 152-8551, Japan}
\affil[26]{Hiroshima Astrophysical Science Center, Hiroshima University, 1-3-1 Kagamiyama, Higashi-Hiroshima, Hiroshima 739-8526, Japan}
\affil[27]{Core Research for Energetic Universe (Core-U), Hiroshima University, 1-3-1 Kagamiyama, Higashi-Hiroshima, Hiroshima 739-8526, Japan}
\affil[28]{Planetary Exploration Research Center, Chiba Institute of Technology 2-17-1 Tsudanuma, Narashino, Chiba 275-0016, Japan}
\affil[29]{Crimean Astrophysical Observatory RAS, P/O Nauchny, 298409, Crimea}
\affil[30]{Universit\'e de Strasbourg, CNRS, Observatoire Astronomique de Strasbourg, UMR 7550, 67000 Strasbourg, France}
\affil[31]{Istituto Nazionale di Fisica Nucleare, Sezione di Torino, Via Pietro Giuria 1, 10125 Torino, Italy}
\affil[32]{Dipartimento di Fisica, Universit\`{a}  degli Studi di Torino, Via Pietro Giuria 1, 10125 Torino, Italy}
\affil[33]{Science and Technology Institute, Universities Space Research Association, Huntsville, AL 35805, USA}
\affil[34]{Astronomical Institute of the Czech Academy of Sciences, Bo\v{c}n\'i­ II 1401/1, 14100 Praha 4, Czech Republic}
\affil[35]{Physics Department and McDonnell Center for the Space Sciences, Washington University in St. Louis, St. Louis, MO 63130, USA}
\affil[36]{International Space Science Institute (ISSI),Hallerstrasse 6, 3012 Bern, Switzerland}
\affil[37]{Dipartimento di Matematica e Fisica, Universit\`{a} degli Studi Roma Tre, Via della Vasca Navale 84, 00146 Roma, Italy}
\affil[38]{Graduate School of Science, Division of Particle and Astrophysical Science, Nagoya University, Furo-cho, Chikusa-ku, Nagoya, Aichi 464-8602, Japan}
\affil[39]{Universit\'e Grenoble Alpes, CNRS, IPAG, 38000 Grenoble, France}
\affil[40]{Mullard Space Science Laboratory, University College London, Holmbury St Mary, Dorking, Surrey RH5 6NT, UK}
\affil[41]{INAF Osservatorio Astronomico di Cagliari, Via della Scienza 5, 09047 Selargius (CA), Italy}
\affil[42]{Istituto Nazionale di Fisica Nucleare, Sezione di Pisa, Largo B. Pontecorvo 3, 56127 Pisa, Italy}
\affil[43]{Dipartimento di Fisica, Universit\`{a}  di Pisa, Largo B. Pontecorvo 3, 56127 Pisa, Italy}
\affil[44]{INAF Osservatorio Astrofisico di Arcetri, Largo Enrico Fermi 5, 50125 Firenze, Italy}
\affil[45]{Dipartimento di Fisica e Astronomia, Universit\`{a}  degli Studi di Firenze, Via Sansone 1, 50019 Sesto Fiorentino (FI), Italy}
\affil[46]{Istituto Nazionale di Fisica Nucleare, Sezione di Firenze, Via Sansone 1, 50019 Sesto Fiorentino (FI), Italy}
\affil[47]{Istituto Nazionale di Fisica Nucleare, Sezione di Roma "Tor Vergata", Via della Ricerca Scientifica 1, 00133 Roma, Italy}
\affil[48]{Institut f\"ur Astronomie und Astrophysik, Universit\"at T\"ubingen, Sand 1, 72076 T\"ubingen, Germany}
\affil[49]{RIKEN Cluster for Pioneering Research, 2-1 Hirosawa, Wako, Saitama 351-0198, Japan}
\affil[50]{California Institute of Technology, Pasadena, CA 91125, USA}
\affil[51]{Yamagata University,1-4-12 Kojirakawa-machi, Yamagata-shi 990-8560, Japan}
\affil[52]{Osaka University, 1-1 Yamadaoka, Suita, Osaka 565-0871, Japan}
\affil[53]{University of British Columbia, Vancouver, BC V6T 1Z4, Canada}
\affil[54]{Department of Physics, Faculty of Science and Engineering, Chuo University, 1-13-27 Kasuga, Bunkyo-ku, Tokyo 112-8551, Japan}
\affil[55]{Department of Physics, The University of Hong Kong, Pokfulam, Hong Kong}
\affil[56]{Department of Astronomy and Astrophysics, Pennsylvania State University, University Park, PA 16802, USA}
\affil[57]{Department of Physics and Astronomy, 20014 University of Turku, Finland}
\affil[58]{Dipartimento di Fisica e Astronomia, Universit\`{a}  degli Studi di Padova, Via Marzolo 8, 35131 Padova, Italy}
\affil[59]{Department of Astronomy, University of Maryland, College Park, Maryland 20742, USA}
\affil[60]{Anton Pannekoek Institute for Astronomy \& GRAPPA, University of Amsterdam, Science Park 904, 1098 XH Amsterdam, The Netherlands}
\affil[61]{Guangxi Key Laboratory for Relativistic Astrophysics, School of Physical Science and Technology, Guangxi University, Nanning 530004, China}

